The Federation Strikes Back: A Survey of Federated Learning Privacy Attacks, Defenses, Applications, and Policy Landscape

Deep learning has shown incredible potential across a wide array of tasks, and accompanied by this growth has been an insatiable appetite for data. However, a large amount of data needed for enabling deep learning is stored on personal devices, and recent concerns on privacy have further highlighted challenges for accessing such data. As a result, federated learning (FL) has emerged as an important privacy-preserving technology that enables collaborative training of machine learning models without the need to send the raw, potentially sensitive, data to a central server. However, the fundamental premise that sending model updates to a server is privacy-preserving only holds if the updates cannot be "reverse engineered" to infer information about the private training data. It has been shown under a wide variety of settings that this privacy premise does not hold. In this survey paper, we provide a comprehensive literature review of the different privacy attacks and defense methods in FL. We identify the current limitations of these attacks and highlight the settings in which the privacy of an FL client can be broken. We further dissect some of the successful industry applications of FL and draw lessons for future successful adoption. We survey the emerging landscape of privacy regulation for FL and conclude with future directions for taking FL toward the cherished goal of generating accurate models while preserving the privacy of the data from its participants.

==> tikzlibraryshadows.code.tex <==
@inproceedings{snp2023,
  title={On the (In) security of Peer-to-Peer Decentralized Machine Learning},
  author={Pasquini, Dario and Raynal, Mathilde and Troncoso, Carmela},
  booktitle={2023 IEEE Symposium on Security and Privacy (SP)},
  pages={418--436},
  year={2023},
  organization={IEEE Computer Society}
}

@inproceedings{hsl,
  title={How to Learn Collaboratively-Federated Learning to Peer-to-Peer Learning and What’s at Stake},
  author={Sharma, Atul and Zhao, Joshua C and Chen, Wei and Qiu, Qiang and Bagchi, Saurabh and Chaterji, Somali},
  booktitle={2023 53rd Annual IEEE/IFIP International Conference on Dependable Systems and Networks-Supplemental Volume (DSN-S)},
  pages={122--126},
  year={2023},
  organization={IEEE}
}

@article{relaysum,
  title={Relaysum for decentralized deep learning on heterogeneous data},
  author={Vogels, Thijs and He, Lie and Koloskova, Anastasiia and Karimireddy, Sai Praneeth and Lin, Tao and Stich, Sebastian U and Jaggi, Martin},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={28004--28015},
  year={2021}
}

@article{networkDP,
  title={Federated multi-task learning under a mixture of distributions},
  author={Marfoq, Othmane and Neglia, Giovanni and Bellet, Aur{\'e}lien and Kameni, Laetitia and Vidal, Richard},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={15434--15447},
  year={2021}
}

@inproceedings{privacyAmplification,
  title={Privacy amplification by decentralization},
  author={Cyffers, Edwige and Bellet, Aur{\'e}lien},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={5334--5353},
  year={2022},
  organization={PMLR}
}

@article{dfl,
  title={Decentralized federated averaging},
  author={Sun, Tao and Li, Dongsheng and Wang, Bao},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={45},
  number={4},
  pages={4289--4301},
  year={2022},
  publisher={IEEE}
}

@article{geiping2020inverting,
  title={Inverting gradients-how easy is it to break privacy in federated learning?},
  author={Geiping, Jonas and Bauermeister, Hartmut and Dr{\"o}ge, Hannah and Moeller, Michael},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={16937--16947},
  year={2020}
}

@inproceedings{membership,
  title={Gan enhanced membership inference: A passive local attack in federated learning},
  author={Zhang, Jingwen and Zhang, Jiale and Chen, Junjun and Yu, Shui},
  booktitle={ICC 2020-2020 IEEE International Conference on Communications (ICC)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

@article{surveyDP,
  title={Differential privacy for deep and federated learning: A survey},
  author={El Ouadrhiri, Ahmed and Abdelhadi, Ahmed},
  journal={IEEE access},
  volume={10},
  pages={22359--22380},
  year={2022},
  publisher={IEEE}
}
